SemML 2.0: Synthesizing Controllers for LTL

Synthesizing a reactive system from specifications given in linear temporal logic (LTL) is a classical problem, finding its applications in safety-critical systems design. These systems are typically represented using either Mealy machines or AIGER circuits. We present the second version of SemML, which outperforms all state-of-the-art tools for finding either solution. Aside from implementing the classical automata-theoretic approach, our tool utilizes partial exploration and machine-learning guidance for obtaining solutions efficiently, and numerous heuristics and improvements of classic algorithms for extracting small representations of these solutions. We evaluate our tool against the existing state-of-the-art tools (in particular Strix, LtlSynt, and the previous version of SemML) on the dataset of the synthesis competition SYNTCOMP. We show that we solve significantly more instances and do so much faster than other tools, while maintaining state-of-the-art solution quality.

==> data/commands.tex <==
\newcommand{\StrixRealSolvesTotal}{1346}
\newcommand{\StrixRealSolvesReal}{610}
\newcommand{\StrixRealSolvesUnreal}{736}
\newcommand{\SemmlRealSolvesTotal}{1412}
\newcommand{\SemmlRealSolvesReal}{640}
\newcommand{\SemmlRealSolvesUnreal}{772}
\newcommand{\SemmlFastRealSolvesTotal}{1412}
\newcommand{\SemmlFastRealSolvesReal}{640}
\newcommand{\SemmlFastRealSolvesUnreal}{772}
\newcommand{\SemmlTacRealSolvesTotal}{1361}
\newcommand{\SemmlTacRealSolvesReal}{619}
\newcommand{\SemmlTacRealSolvesUnreal}{742}
\newcommand{\LtlsyntRealSolvesTotal}{1319}
\newcommand{\LtlsyntRealSolvesReal}{610}
\newcommand{\LtlsyntRealSolvesUnreal}{709}
\newcommand{\StrixMealySolvesTotal}{1314}
\newcommand{\StrixMealySolvesReal}{578}
\newcommand{\StrixMealySolvesUnreal}{736}
\newcommand{\StrixMealyTimeTotalinh}{139}
\newcommand{\StrixMealyTimeMeanins}{321.42}
\newcommand{\SemmlMealySolvesTotal}{1391}
\newcommand{\SemmlMealySolvesReal}{617}
\newcommand{\SemmlMealySolvesUnreal}{774}
\newcommand{\SemmlMealyTimeTotalinh}{101}
\newcommand{\SemmlMealyTimeMeanins}{233.70}
\newcommand{\SemmlFastMealySolvesTotal}{1398}
\newcommand{\SemmlFastMealySolvesReal}{625}
\newcommand{\SemmlFastMealySolvesUnreal}{773}
\newcommand{\SemmlFastMealyTimeTotalinh}{96}
\newcommand{\SemmlFastMealyTimeMeanins}{222.58}
\newcommand{\LtlsyntMealySolvesTotal}{1204}
\newcommand{\LtlsyntMealySolvesReal}{495}
\newcommand{\LtlsyntMealySolvesUnreal}{709}
\newcommand{\LtlsyntMealyTimeTotalinh}{189}
\newcommand{\LtlsyntMealyTimeMeanins}{437.30}
\newcommand{\StrixAigerSolvesTotal}{1330}
\newcommand{\StrixAigerSolvesReal}{594}
\newcommand{\StrixAigerSolvesUnreal}{736}
\newcommand{\StrixAigerTimeTotalinh}{134}
\newcommand{\StrixAigerTimeMeanins}{310.49}
\newcommand{\SemmlAigerSolvesTotal}{1375}
\newcommand{\SemmlAigerSolvesReal}{603}
\newcommand{\SemmlAigerSolvesUnreal}{772}
\newcommand{\SemmlAigerTimeTotalinh}{111}
\newcommand{\SemmlAigerTimeMeanins}{256.15}
\newcommand{\SemmlFastAigerSolvesTotal}{1392}
\newcommand{\SemmlFastAigerSolvesReal}{618}
\newcommand{\SemmlFastAigerSolvesUnreal}{774}
\newcommand{\SemmlFastAigerTimeTotalinh}{101}
\newcommand{\SemmlFastAigerTimeMeanins}{234.49}
\newcommand{\SemmlTacAigerSolvesTotal}{1273}
\newcommand{\SemmlTacAigerSolvesReal}{531}
\newcommand{\SemmlTacAigerSolvesUnreal}{742}
\newcommand{\SemmlTacAigerTimeTotalinh}{163}
\newcommand{\SemmlTacAigerTimeMeanins}{375.93}
\newcommand{\LtlsyntAigerSolvesTotal}{1213}
\newcommand{\LtlsyntAigerSolvesReal}{504}
\newcommand{\LtlsyntAigerSolvesUnreal}{709}
\newcommand{\LtlsyntAigerTimeTotalinh}{184}
\newcommand{\LtlsyntAigerTimeMeanins}{425.79}
\newcommand{\StrixMealyScoresTotal}{980.17}
\newcommand{\StrixMealyScoresMean}{1.70}
\newcommand{\SemmlMealyScoresTotal}{1182.48}
\newcommand{\SemmlMealyScoresMean}{1.92}
\newcommand{\SemmlFastMealyScoresTotal}{1092.66}
\newcommand{\SemmlFastMealyScoresMean}{1.75}
\newcommand{\LtlsyntMealyScoresTotal}{830.88}
\newcommand{\LtlsyntMealyScoresMean}{1.68}
\newcommand{\StrixAigerScoresTotal}{1101.51}
\newcommand{\StrixAigerScoresMean}{1.85}
\newcommand{\SemmlAigerScoresTotal}{1098.47}
\newcommand{\SemmlAigerScoresMean}{1.82}
\newcommand{\SemmlFastAigerScoresTotal}{981.05}
\newcommand{\SemmlFastAigerScoresMean}{1.59}
\newcommand{\SemmlTacAigerScoresTotal}{731.56}
\newcommand{\SemmlTacAigerScoresMean}{1.38}
\newcommand{\LtlsyntAigerScoresTotal}{646.77}
\newcommand{\LtlsyntAigerScoresMean}{1.28}
\newcommand{\SemmlStrixRealUniqueSolvesTotal}{70}
\newcommand{\SemmlStrixRealUniqueSolvesReal}{34}
\newcommand{\SemmlStrixRealUniqueSolvesUnreal}{36}
\newcommand{\StrixSemmlRealUniqueSolvesTotal}{4}
\newcommand{\StrixSemmlRealUniqueSolvesReal}{4}
\newcommand{\StrixSemmlRealUniqueSolvesUnreal}{0}
\newcommand{\SemmlStrixRealSolvesBoth}{1342}
\newcommand{\SemmlStrixRealSolvesNeither}{147}
\newcommand{\SemmlStrixRealTimeMeanZero}{5.33}
\newcommand{\SemmlStrixRealTimeMeanFive}{0.74}
\newcommand{\SemmlStrixRealTimeMeanTen}{0.46}
\newcommand{\SemmlStrixRealTimeMeanThirty}{0.35}
\newcommand{\SemmlStrixRealTimeMeanOneTwenty}{0.25}
\newcommand{\SemmlStrixRealTimeWtoMeanZero}{4.33}
\newcommand{\SemmlStrixRealTimeWtoMeanFive}{0.59}
\newcommand{\SemmlStrixRealTimeWtoMeanTen}{0.35}
\newcommand{\SemmlStrixRealTimeWtoMeanThirty}{0.26}
\newcommand{\SemmlStrixRealTimeWtoMeanOneTwenty}{0.17}
\newcommand{\SemmlStrixRealTimeFacZero}{0.19}
\newcommand{\SemmlStrixRealTimeFacFive}{1.35}
\newcommand{\SemmlStrixRealTimeFacTen}{2.18}
\newcommand{\SemmlStrixRealTimeFacThirty}{2.88}
\newcommand{\SemmlStrixRealTimeFacOneTwenty}{3.93}
\newcommand{\SemmlStrixRealTimeWtoFacZero}{0.23}
\newcommand{\SemmlStrixRealTimeWtoFacFive}{1.70}
\newcommand{\SemmlStrixRealTimeWtoFacTen}{2.82}
\newcommand{\SemmlStrixRealTimeWtoFacThirty}{3.88}
\newcommand{\SemmlStrixRealTimeWtoFacOneTwenty}{5.84}
\newcommand{\SemmlStrixRealTimeMeanNZero}{1342}
\newcommand{\SemmlStrixRealTimeMeanNFive}{559}
\newcommand{\SemmlStrixRealTimeMeanNTen}{367}
\newcommand{\SemmlStrixRealTimeMeanNThirty}{238}
\newcommand{\SemmlStrixRealTimeMeanNOneTwenty}{102}
\newcommand{\SemmlStrixRealTimeWtoMeanNZero}{1416}
\newcommand{\SemmlStrixRealTimeWtoMeanNFive}{633}
\newcommand{\SemmlStrixRealTimeWtoMeanNTen}{441}
\newcommand{\SemmlStrixRealTimeWtoMeanNThirty}{312}
\newcommand{\SemmlStrixRealTimeWtoMeanNOneTwenty}{176}
\newcommand{\SemmlSemmlTacRealUniqueSolvesTotal}{58}
\newcommand{\SemmlSemmlTacRealUniqueSolvesReal}{25}
\newcommand{\SemmlSemmlTacRealUniqueSolvesUnreal}{33}
\newcommand{\SemmlTacSemmlRealUniqueSolvesTotal}{7}
\newcommand{\SemmlTacSemmlRealUniqueSolvesReal}{4}
\newcommand{\SemmlTacSemmlRealUniqueSolvesUnreal}{3}
\newcommand{\SemmlSemmlTacRealSolvesBoth}{1354}
\newcommand{\SemmlSemmlTacRealSolvesNeither}{144}
\newcommand{\SemmlSemmlTacRealTimeMeanZero}{1.10}
\newcommand{\SemmlSemmlTacRealTimeMeanFive}{0.95}
\newcommand{\SemmlSemmlTacRealTimeMeanTen}{0.85}
\newcommand{\SemmlSemmlTacRealTimeMeanThirty}{0.74}
\newcommand{\SemmlSemmlTacRealTimeMeanOneTwenty}{0.66}
\newcommand{\SemmlSemmlTacRealTimeWtoMeanZero}{0.97}
\newcommand{\SemmlSemmlTacRealTimeWtoMeanFive}{0.73}
\newcommand{\SemmlSemmlTacRealTimeWtoMeanTen}{0.57}
\newcommand{\SemmlSemmlTacRealTimeWtoMeanThirty}{0.38}
\newcommand{\SemmlSemmlTacRealTimeWtoMeanOneTwenty}{0.23}
\newcommand{\SemmlSemmlTacRealTimeFacZero}{0.91}
\newcommand{\SemmlSemmlTacRealTimeFacFive}{1.05}
\newcommand{\SemmlSemmlTacRealTimeFacTen}{1.17}
\newcommand{\SemmlSemmlTacRealTimeFacThirty}{1.34}
\newcommand{\SemmlSemmlTacRealTimeFacOneTwenty}{1.51}
\newcommand{\SemmlSemmlTacRealTimeWtoFacZero}{1.03}
\newcommand{\SemmlSemmlTacRealTimeWtoFacFive}{1.37}
\newcommand{\SemmlSemmlTacRealTimeWtoFacTen}{1.74}
\newcommand{\SemmlSemmlTacRealTimeWtoFacThirty}{2.62}
\newcommand{\SemmlSemmlTacRealTimeWtoFacOneTwenty}{4.36}
\newcommand{\SemmlSemmlTacRealTimeMeanNZero}{1354}
\newcommand{\SemmlSemmlTacRealTimeMeanNFive}{596}
\newcommand{\SemmlSemmlTacRealTimeMeanNTen}{351}
\newcommand{\SemmlSemmlTacRealTimeMeanNThirty}{170}
\newcommand{\SemmlSemmlTacRealTimeMeanNOneTwenty}{80}
\newcommand{\SemmlSemmlTacRealTimeWtoMeanNZero}{1419}
\newcommand{\SemmlSemmlTacRealTimeWtoMeanNFive}{661}
\newcommand{\SemmlSemmlTacRealTimeWtoMeanNTen}{416}
\newcommand{\SemmlSemmlTacRealTimeWtoMeanNThirty}{235}
\newcommand{\SemmlSemmlTacRealTimeWtoMeanNOneTwenty}{143}
\newcommand{\SemmlSemmlFastRealUniqueSolvesTotal}{0}
\newcommand{\SemmlSemmlFastRealUniqueSolvesReal}{0}
\newcommand{\SemmlSemmlFastRealUniqueSolvesUnreal}{0}
\newcommand{\SemmlFastSemmlRealUniqueSolvesTotal}{0}
\newcommand{\SemmlFastSemmlRealUniqueSolvesReal}{0}
\newcommand{\SemmlFastSemmlRealUniqueSolvesUnreal}{0}
\newcommand{\SemmlSemmlFastRealSolvesBoth}{1412}
\newcommand{\SemmlSemmlFastRealSolvesNeither}{151}
\newcommand{\SemmlSemmlFastRealTimeMeanZero}{1.00}
\newcommand{\SemmlSemmlFastRealTimeMeanFive}{1.00}
\newcommand{\SemmlSemmlFastRealTimeMeanTen}{1.00}
\newcommand{\SemmlSemmlFastRealTimeMeanThirty}{1.00}
\newcommand{\SemmlSemmlFastRealTimeMeanOneTwenty}{1.00}
\newcommand{\SemmlSemmlFastRealTimeWtoMeanZero}{1.00}
\newcommand{\SemmlSemmlFastRealTimeWtoMeanFive}{1.00}
\newcommand{\SemmlSemmlFastRealTimeWtoMeanTen}{1.00}
\newcommand{\SemmlSemmlFastRealTimeWtoMeanThirty}{1.00}
\newcommand{\SemmlSemmlFastRealTimeWtoMeanOneTwenty}{1.00}
\newcommand{\SemmlSemmlFastRealTimeFacZero}{1.00}
\newcommand{\SemmlSemmlFastRealTimeFacFive}{1.00}
\newcommand{\SemmlSemmlFastRealTimeFacTen}{1.00}
\newcommand{\SemmlSemmlFastRealTimeFacThirty}{1.00}
\newcommand{\SemmlSemmlFastRealTimeFacOneTwenty}{1.00}
\newcommand{\SemmlSemmlFastRealTimeWtoFacZero}{1.00}
\newcommand{\SemmlSemmlFastRealTimeWtoFacFive}{1.00}
\newcommand{\SemmlSemmlFastRealTimeWtoFacTen}{1.00}
\newcommand{\SemmlSemmlFastRealTimeWtoFacThirty}{1.00}
\newcommand{\SemmlSemmlFastRealTimeWtoFacOneTwenty}{1.00}
\newcommand{\SemmlSemmlFastRealTimeMeanNZero}{1412}
\newcommand{\SemmlSemmlFastRealTimeMeanNFive}{617}
\newcommand{\SemmlSemmlFastRealTimeMeanNTen}{371}
\newcommand{\SemmlSemmlFastRealTimeMeanNThirty}{175}
\newcommand{\SemmlSemmlFastRealTimeMeanNOneTwenty}{84}
\newcommand{\SemmlSemmlFastRealTimeWtoMeanNZero}{1412}
\newcommand{\SemmlSemmlFastRealTimeWtoMeanNFive}{617}
\newcommand{\SemmlSemmlFastRealTimeWtoMeanNTen}{371}
\newcommand{\SemmlSemmlFastRealTimeWtoMeanNThirty}{175}
\newcommand{\SemmlSemmlFastRealTimeWtoMeanNOneTwenty}{84}
\newcommand{\SemmlLtlsyntRealUniqueSolvesTotal}{136}
\newcommand{\SemmlLtlsyntRealUniqueSolvesReal}{71}
\newcommand{\SemmlLtlsyntRealUniqueSolvesUnreal}{65}
\newcommand{\LtlsyntSemmlRealUniqueSolvesTotal}{43}
\newcommand{\LtlsyntSemmlRealUniqueSolvesReal}{41}
\newcommand{\LtlsyntSemmlRealUniqueSolvesUnreal}{2}
\newcommand{\SemmlLtlsyntRealSolvesBoth}{1276}
\newcommand{\SemmlLtlsyntRealSolvesNeither}{108}
\newcommand{\SemmlLtlsyntRealTimeMeanZero}{26.28}
\newcommand{\SemmlLtlsyntRealTimeMeanFive}{7.65}
\newcommand{\SemmlLtlsyntRealTimeMeanTen}{3.29}
\newcommand{\SemmlLtlsyntRealTimeMeanThirty}{1.24}
\newcommand{\SemmlLtlsyntRealTimeMeanOneTwenty}{1.39}
\newcommand{\SemmlLtlsyntRealTimeWtoMeanZero}{16.68}
\newcommand{\SemmlLtlsyntRealTimeWtoMeanFive}{4.00}
\newcommand{\SemmlLtlsyntRealTimeWtoMeanTen}{1.70}
\newcommand{\SemmlLtlsyntRealTimeWtoMeanThirty}{0.81}
\newcommand{\SemmlLtlsyntRealTimeWtoMeanOneTwenty}{0.68}
\newcommand{\SemmlLtlsyntRealTimeFacZero}{0.04}
\newcommand{\SemmlLtlsyntRealTimeFacFive}{0.13}
\newcommand{\SemmlLtlsyntRealTimeFacTen}{0.30}
\newcommand{\SemmlLtlsyntRealTimeFacThirty}{0.80}
\newcommand{\SemmlLtlsyntRealTimeFacOneTwenty}{0.72}
\newcommand{\SemmlLtlsyntRealTimeWtoFacZero}{0.06}
\newcommand{\SemmlLtlsyntRealTimeWtoFacFive}{0.25}
\newcommand{\SemmlLtlsyntRealTimeWtoFacTen}{0.59}
\newcommand{\SemmlLtlsyntRealTimeWtoFacThirty}{1.23}
\newcommand{\SemmlLtlsyntRealTimeWtoFacOneTwenty}{1.46}
\newcommand{\SemmlLtlsyntRealTimeMeanNZero}{1276}
\newcommand{\SemmlLtlsyntRealTimeMeanNFive}{500}
\newcommand{\SemmlLtlsyntRealTimeMeanNTen}{291}
\newcommand{\SemmlLtlsyntRealTimeMeanNThirty}{150}
\newcommand{\SemmlLtlsyntRealTimeMeanNOneTwenty}{76}
\newcommand{\SemmlLtlsyntRealTimeWtoMeanNZero}{1455}
\newcommand{\SemmlLtlsyntRealTimeWtoMeanNFive}{679}
\newcommand{\SemmlLtlsyntRealTimeWtoMeanNTen}{463}
\newcommand{\SemmlLtlsyntRealTimeWtoMeanNThirty}{322}
\newcommand{\SemmlLtlsyntRealTimeWtoMeanNOneTwenty}{245}
\newcommand{\SemmlStrixMealyUniqueSolvesTotal}{79}
\newcommand{\SemmlStrixMealyUniqueSolvesReal}{41}
\newcommand{\SemmlStrixMealyUniqueSolvesUnreal}{38}
\newcommand{\StrixSemmlMealyUniqueSolvesTotal}{2}
\newcommand{\StrixSemmlMealyUniqueSolvesReal}{2}
\newcommand{\StrixSemmlMealyUniqueSolvesUnreal}{0}
\newcommand{\SemmlStrixMealySolvesBoth}{1312}
\newcommand{\SemmlStrixMealySolvesNeither}{170}
\newcommand{\SemmlStrixMealyTimeMeanZero}{5.40}
\newcommand{\SemmlStrixMealyTimeMeanFive}{1.01}
\newcommand{\SemmlStrixMealyTimeMeanTen}{0.52}
\newcommand{\SemmlStrixMealyTimeMeanThirty}{0.38}
\newcommand{\SemmlStrixMealyTimeMeanOneTwenty}{0.25}
\newcommand{\SemmlStrixMealyTimeWtoMeanZero}{4.29}
\newcommand{\SemmlStrixMealyTimeWtoMeanFive}{0.77}
\newcommand{\SemmlStrixMealyTimeWtoMeanTen}{0.39}
\newcommand{\SemmlStrixMealyTimeWtoMeanThirty}{0.27}
\newcommand{\SemmlStrixMealyTimeWtoMeanOneTwenty}{0.17}
\newcommand{\SemmlStrixMealyTimeFacZero}{0.19}
\newcommand{\SemmlStrixMealyTimeFacFive}{0.99}
\newcommand{\SemmlStrixMealyTimeFacTen}{1.91}
\newcommand{\SemmlStrixMealyTimeFacThirty}{2.66}
\newcommand{\SemmlStrixMealyTimeFacOneTwenty}{4.03}
\newcommand{\SemmlStrixMealyTimeWtoFacZero}{0.23}
\newcommand{\SemmlStrixMealyTimeWtoFacFive}{1.30}
\newcommand{\SemmlStrixMealyTimeWtoFacTen}{2.56}
\newcommand{\SemmlStrixMealyTimeWtoFacThirty}{3.71}
\newcommand{\SemmlStrixMealyTimeWtoFacOneTwenty}{5.98}
\newcommand{\SemmlStrixMealyTimeMeanNZero}{1312}
\newcommand{\SemmlStrixMealyTimeMeanNFive}{597}
\newcommand{\SemmlStrixMealyTimeMeanNTen}{368}
\newcommand{\SemmlStrixMealyTimeMeanNThirty}{234}
\newcommand{\SemmlStrixMealyTimeMeanNOneTwenty}{98}
\newcommand{\SemmlStrixMealyTimeWtoMeanNZero}{1393}
\newcommand{\SemmlStrixMealyTimeWtoMeanNFive}{678}
\newcommand{\SemmlStrixMealyTimeWtoMeanNTen}{449}
\newcommand{\SemmlStrixMealyTimeWtoMeanNThirty}{315}
\newcommand{\SemmlStrixMealyTimeWtoMeanNOneTwenty}{179}
\newcommand{\SemmlStrixMealySizeMeanTotal}{0.77}
\newcommand{\SemmlStrixMealySizeMeanReal}{0.60}
\newcommand{\SemmlStrixMealySizeMeanNTotal}{1287}
\newcommand{\SemmlStrixMealySizeMeanNReal}{576}
\newcommand{\SemmlSemmlFastMealyUniqueSolvesTotal}{1}
\newcommand{\SemmlSemmlFastMealyUniqueSolvesReal}{0}
\newcommand{\SemmlSemmlFastMealyUniqueSolvesUnreal}{1}
\newcommand{\SemmlFastSemmlMealyUniqueSolvesTotal}{8}
\newcommand{\SemmlFastSemmlMealyUniqueSolvesReal}{8}
\newcommand{\SemmlFastSemmlMealyUniqueSolvesUnreal}{0}
\newcommand{\SemmlSemmlFastMealySolvesBoth}{1390}
\newcommand{\SemmlSemmlFastMealySolvesNeither}{164}
\newcommand{\SemmlSemmlFastMealyTimeMeanZero}{1.10}
\newcommand{\SemmlSemmlFastMealyTimeMeanFive}{1.17}
\newcommand{\SemmlSemmlFastMealyTimeMeanTen}{1.22}
\newcommand{\SemmlSemmlFastMealyTimeMeanThirty}{1.39}
\newcommand{\SemmlSemmlFastMealyTimeMeanOneTwenty}{1.53}
\newcommand{\SemmlSemmlFastMealyTimeWtoMeanZero}{1.11}
\newcommand{\SemmlSemmlFastMealyTimeWtoMeanFive}{1.18}
\newcommand{\SemmlSemmlFastMealyTimeWtoMeanTen}{1.24}
\newcommand{\SemmlSemmlFastMealyTimeWtoMeanThirty}{1.43}
\newcommand{\SemmlSemmlFastMealyTimeWtoMeanOneTwenty}{1.59}
\newcommand{\SemmlSemmlFastMealyTimeFacZero}{0.91}
\newcommand{\SemmlSemmlFastMealyTimeFacFive}{0.86}
\newcommand{\SemmlSemmlFastMealyTimeFacTen}{0.82}
\newcommand{\SemmlSemmlFastMealyTimeFacThirty}{0.72}
\newcommand{\SemmlSemmlFastMealyTimeFacOneTwenty}{0.65}
\newcommand{\SemmlSemmlFastMealyTimeWtoFacZero}{0.90}
\newcommand{\SemmlSemmlFastMealyTimeWtoFacFive}{0.85}
\newcommand{\SemmlSemmlFastMealyTimeWtoFacTen}{0.80}
\newcommand{\SemmlSemmlFastMealyTimeWtoFacThirty}{0.70}
\newcommand{\SemmlSemmlFastMealyTimeWtoFacOneTwenty}{0.63}
\newcommand{\SemmlSemmlFastMealyTimeMeanNZero}{1390}
\newcommand{\SemmlSemmlFastMealyTimeMeanNFive}{666}
\newcommand{\SemmlSemmlFastMealyTimeMeanNTen}{383}
\newcommand{\SemmlSemmlFastMealyTimeMeanNThirty}{185}
\newcommand{\SemmlSemmlFastMealyTimeMeanNOneTwenty}{88}
\newcommand{\SemmlSemmlFastMealyTimeWtoMeanNZero}{1399}
\newcommand{\SemmlSemmlFastMealyTimeWtoMeanNFive}{675}
\newcommand{\SemmlSemmlFastMealyTimeWtoMeanNTen}{392}
\newcommand{\SemmlSemmlFastMealyTimeWtoMeanNThirty}{194}
\newcommand{\SemmlSemmlFastMealyTimeWtoMeanNOneTwenty}{96}
\newcommand{\SemmlSemmlFastMealySizeMeanTotal}{0.84}
\newcommand{\SemmlSemmlFastMealySizeMeanReal}{0.68}
\newcommand{\SemmlSemmlFastMealySizeMeanNTotal}{1361}
\newcommand{\SemmlSemmlFastMealySizeMeanNReal}{617}
\newcommand{\SemmlLtlsyntMealyUniqueSolvesTotal}{202}
\newcommand{\SemmlLtlsyntMealyUniqueSolvesReal}{135}
\newcommand{\SemmlLtlsyntMealyUniqueSolvesUnreal}{67}
\newcommand{\LtlsyntSemmlMealyUniqueSolvesTotal}{15}
\newcommand{\LtlsyntSemmlMealyUniqueSolvesReal}{13}
\newcommand{\LtlsyntSemmlMealyUniqueSolvesUnreal}{2}
\newcommand{\SemmlLtlsyntMealySolvesBoth}{1189}
\newcommand{\SemmlLtlsyntMealySolvesNeither}{157}
\newcommand{\SemmlLtlsyntMealyTimeMeanZero}{23.64}
\newcommand{\SemmlLtlsyntMealyTimeMeanFive}{7.21}
\newcommand{\SemmlLtlsyntMealyTimeMeanTen}{2.53}
\newcommand{\SemmlLtlsyntMealyTimeMeanThirty}{0.83}
\newcommand{\SemmlLtlsyntMealyTimeMeanOneTwenty}{0.66}
\newcommand{\SemmlLtlsyntMealyTimeWtoMeanZero}{9.02}
\newcommand{\SemmlLtlsyntMealyTimeWtoMeanFive}{1.61}
\newcommand{\SemmlLtlsyntMealyTimeWtoMeanTen}{0.42}
\newcommand{\SemmlLtlsyntMealyTimeWtoMeanThirty}{0.14}
\newcommand{\SemmlLtlsyntMealyTimeWtoMeanOneTwenty}{0.08}
\newcommand{\SemmlLtlsyntMealyTimeFacZero}{0.04}
\newcommand{\SemmlLtlsyntMealyTimeFacFive}{0.14}
\newcommand{\SemmlLtlsyntMealyTimeFacTen}{0.40}
\newcommand{\SemmlLtlsyntMealyTimeFacThirty}{1.20}
\newcommand{\SemmlLtlsyntMealyTimeFacOneTwenty}{1.51}
\newcommand{\SemmlLtlsyntMealyTimeWtoFacZero}{0.11}
\newcommand{\SemmlLtlsyntMealyTimeWtoFacFive}{0.62}
\newcommand{\SemmlLtlsyntMealyTimeWtoFacTen}{2.36}
\newcommand{\SemmlLtlsyntMealyTimeWtoFacThirty}{7.33}
\newcommand{\SemmlLtlsyntMealyTimeWtoFacOneTwenty}{13.03}
\newcommand{\SemmlLtlsyntMealyTimeMeanNZero}{1189}
\newcommand{\SemmlLtlsyntMealyTimeMeanNFive}{513}
\newcommand{\SemmlLtlsyntMealyTimeMeanNTen}{285}
\newcommand{\SemmlLtlsyntMealyTimeMeanNThirty}{150}
\newcommand{\SemmlLtlsyntMealyTimeMeanNOneTwenty}{74}
\newcommand{\SemmlLtlsyntMealyTimeWtoMeanNZero}{1406}
\newcommand{\SemmlLtlsyntMealyTimeWtoMeanNFive}{730}
\newcommand{\SemmlLtlsyntMealyTimeWtoMeanNTen}{495}
\newcommand{\SemmlLtlsyntMealyTimeWtoMeanNThirty}{360}
\newcommand{\SemmlLtlsyntMealyTimeWtoMeanNOneTwenty}{283}
\newcommand{\SemmlLtlsyntMealySizeMeanTotal}{0.58}
\newcommand{\SemmlLtlsyntMealySizeMeanReal}{0.58}
\newcommand{\SemmlLtlsyntMealySizeMeanNTotal}{482}
\newcommand{\SemmlLtlsyntMealySizeMeanNReal}{482}
\newcommand{\SemmlStrixAigerUniqueSolvesTotal}{64}
\newcommand{\SemmlStrixAigerUniqueSolvesReal}{28}
\newcommand{\SemmlStrixAigerUniqueSolvesUnreal}{36}
\newcommand{\StrixSemmlAigerUniqueSolvesTotal}{19}
\newcommand{\StrixSemmlAigerUniqueSolvesReal}{19}
\newcommand{\StrixSemmlAigerUniqueSolvesUnreal}{0}
\newcommand{\SemmlStrixAigerSolvesBoth}{1311}
\newcommand{\SemmlStrixAigerSolvesNeither}{169}
\newcommand{\SemmlStrixAigerTimeMeanZero}{2.79}
\newcommand{\SemmlStrixAigerTimeMeanFive}{0.83}
\newcommand{\SemmlStrixAigerTimeMeanTen}{0.53}
\newcommand{\SemmlStrixAigerTimeMeanThirty}{0.43}
\newcommand{\SemmlStrixAigerTimeMeanOneTwenty}{0.40}
\newcommand{\SemmlStrixAigerTimeWtoMeanZero}{2.44}
\newcommand{\SemmlStrixAigerTimeWtoMeanFive}{0.74}
\newcommand{\SemmlStrixAigerTimeWtoMeanTen}{0.48}
\newcommand{\SemmlStrixAigerTimeWtoMeanThirty}{0.39}
\newcommand{\SemmlStrixAigerTimeWtoMeanOneTwenty}{0.35}
\newcommand{\SemmlStrixAigerTimeFacZero}{0.36}
\newcommand{\SemmlStrixAigerTimeFacFive}{1.20}
\newcommand{\SemmlStrixAigerTimeFacTen}{1.89}
\newcommand{\SemmlStrixAigerTimeFacThirty}{2.34}
\newcommand{\SemmlStrixAigerTimeFacOneTwenty}{2.50}
\newcommand{\SemmlStrixAigerTimeWtoFacZero}{0.41}
\newcommand{\SemmlStrixAigerTimeWtoFacFive}{1.35}
\newcommand{\SemmlStrixAigerTimeWtoFacTen}{2.08}
\newcommand{\SemmlStrixAigerTimeWtoFacThirty}{2.56}
\newcommand{\SemmlStrixAigerTimeWtoFacOneTwenty}{2.85}
\newcommand{\SemmlStrixAigerTimeMeanNZero}{1311}
\newcommand{\SemmlStrixAigerTimeMeanNFive}{646}
\newcommand{\SemmlStrixAigerTimeMeanNTen}{421}
\newcommand{\SemmlStrixAigerTimeMeanNThirty}{257}
\newcommand{\SemmlStrixAigerTimeMeanNOneTwenty}{112}
\newcommand{\SemmlStrixAigerTimeWtoMeanNZero}{1394}
\newcommand{\SemmlStrixAigerTimeWtoMeanNFive}{729}
\newcommand{\SemmlStrixAigerTimeWtoMeanNTen}{504}
\newcommand{\SemmlStrixAigerTimeWtoMeanNThirty}{340}
\newcommand{\SemmlStrixAigerTimeWtoMeanNOneTwenty}{195}
\newcommand{\SemmlStrixAigerSizeMeanTotal}{1.08}
\newcommand{\SemmlStrixAigerSizeMeanReal}{1.08}
\newcommand{\SemmlStrixAigerSizeMeanNTotal}{575}
\newcommand{\SemmlStrixAigerSizeMeanNReal}{575}
\newcommand{\SemmlSemmlTacAigerUniqueSolvesTotal}{107}
\newcommand{\SemmlSemmlTacAigerUniqueSolvesReal}{74}
\newcommand{\SemmlSemmlTacAigerUniqueSolvesUnreal}{33}
\newcommand{\SemmlTacSemmlAigerUniqueSolvesTotal}{5}
\newcommand{\SemmlTacSemmlAigerUniqueSolvesReal}{2}
\newcommand{\SemmlTacSemmlAigerUniqueSolvesUnreal}{3}
\newcommand{\SemmlSemmlTacAigerSolvesBoth}{1268}
\newcommand{\SemmlSemmlTacAigerSolvesNeither}{183}
\newcommand{\SemmlSemmlTacAigerTimeMeanZero}{0.73}
\newcommand{\SemmlSemmlTacAigerTimeMeanFive}{0.59}
\newcommand{\SemmlSemmlTacAigerTimeMeanTen}{0.46}
\newcommand{\SemmlSemmlTacAigerTimeMeanThirty}{0.31}
\newcommand{\SemmlSemmlTacAigerTimeMeanOneTwenty}{0.22}
\newcommand{\SemmlSemmlTacAigerTimeWtoMeanZero}{0.61}
\newcommand{\SemmlSemmlTacAigerTimeWtoMeanFive}{0.45}
\newcommand{\SemmlSemmlTacAigerTimeWtoMeanTen}{0.32}
\newcommand{\SemmlSemmlTacAigerTimeWtoMeanThirty}{0.18}
\newcommand{\SemmlSemmlTacAigerTimeWtoMeanOneTwenty}{0.11}
\newcommand{\SemmlSemmlTacAigerTimeFacZero}{1.36}
\newcommand{\SemmlSemmlTacAigerTimeFacFive}{1.71}
\newcommand{\SemmlSemmlTacAigerTimeFacTen}{2.17}
\newcommand{\SemmlSemmlTacAigerTimeFacThirty}{3.27}
\newcommand{\SemmlSemmlTacAigerTimeFacOneTwenty}{4.63}
\newcommand{\SemmlSemmlTacAigerTimeWtoFacZero}{1.65}
\newcommand{\SemmlSemmlTacAigerTimeWtoFacFive}{2.20}
\newcommand{\SemmlSemmlTacAigerTimeWtoFacTen}{3.16}
\newcommand{\SemmlSemmlTacAigerTimeWtoFacThirty}{5.59}
\newcommand{\SemmlSemmlTacAigerTimeWtoFacOneTwenty}{8.95}
\newcommand{\SemmlSemmlTacAigerTimeMeanNZero}{1268}
\newcommand{\SemmlSemmlTacAigerTimeMeanNFive}{842}
\newcommand{\SemmlSemmlTacAigerTimeMeanNTen}{459}
\newcommand{\SemmlSemmlTacAigerTimeMeanNThirty}{204}
\newcommand{\SemmlSemmlTacAigerTimeMeanNOneTwenty}{95}
\newcommand{\SemmlSemmlTacAigerTimeWtoMeanNZero}{1380}
\newcommand{\SemmlSemmlTacAigerTimeWtoMeanNFive}{954}
\newcommand{\SemmlSemmlTacAigerTimeWtoMeanNTen}{571}
\newcommand{\SemmlSemmlTacAigerTimeWtoMeanNThirty}{316}
\newcommand{\SemmlSemmlTacAigerTimeWtoMeanNOneTwenty}{205}
\newcommand{\SemmlSemmlTacAigerSizeMeanTotal}{0.34}
\newcommand{\SemmlSemmlTacAigerSizeMeanReal}{0.34}
\newcommand{\SemmlSemmlTacAigerSizeMeanNTotal}{529}
\newcommand{\SemmlSemmlTacAigerSizeMeanNReal}{529}
\newcommand{\SemmlSemmlFastAigerUniqueSolvesTotal}{0}
\newcommand{\SemmlSemmlFastAigerUniqueSolvesReal}{0}
\newcommand{\SemmlSemmlFastAigerUniqueSolvesUnreal}{0}
\newcommand{\SemmlFastSemmlAigerUniqueSolvesTotal}{17}
\newcommand{\SemmlFastSemmlAigerUniqueSolvesReal}{15}
\newcommand{\SemmlFastSemmlAigerUniqueSolvesUnreal}{2}
\newcommand{\SemmlSemmlFastAigerSolvesBoth}{1375}
\newcommand{\SemmlSemmlFastAigerSolvesNeither}{171}
\newcommand{\SemmlSemmlFastAigerTimeMeanZero}{1.08}
\newcommand{\SemmlSemmlFastAigerTimeMeanFive}{1.12}
\newcommand{\SemmlSemmlFastAigerTimeMeanTen}{1.17}
\newcommand{\SemmlSemmlFastAigerTimeMeanThirty}{1.31}
\newcommand{\SemmlSemmlFastAigerTimeMeanOneTwenty}{1.49}
\newcommand{\SemmlSemmlFastAigerTimeWtoMeanZero}{1.10}
\newcommand{\SemmlSemmlFastAigerTimeWtoMeanFive}{1.18}
\newcommand{\SemmlSemmlFastAigerTimeWtoMeanTen}{1.27}
\newcommand{\SemmlSemmlFastAigerTimeWtoMeanThirty}{1.54}
\newcommand{\SemmlSemmlFastAigerTimeWtoMeanOneTwenty}{1.97}
\newcommand{\SemmlSemmlFastAigerTimeFacZero}{0.93}
\newcommand{\SemmlSemmlFastAigerTimeFacFive}{0.89}
\newcommand{\SemmlSemmlFastAigerTimeFacTen}{0.86}
\newcommand{\SemmlSemmlFastAigerTimeFacThirty}{0.76}
\newcommand{\SemmlSemmlFastAigerTimeFacOneTwenty}{0.67}
\newcommand{\SemmlSemmlFastAigerTimeWtoFacZero}{0.91}
\newcommand{\SemmlSemmlFastAigerTimeWtoFacFive}{0.85}
\newcommand{\SemmlSemmlFastAigerTimeWtoFacTen}{0.79}
\newcommand{\SemmlSemmlFastAigerTimeWtoFacThirty}{0.65}
\newcommand{\SemmlSemmlFastAigerTimeWtoFacOneTwenty}{0.51}
\newcommand{\SemmlSemmlFastAigerTimeMeanNZero}{1375}
\newcommand{\SemmlSemmlFastAigerTimeMeanNFive}{687}
\newcommand{\SemmlSemmlFastAigerTimeMeanNTen}{399}
\newcommand{\SemmlSemmlFastAigerTimeMeanNThirty}{188}
\newcommand{\SemmlSemmlFastAigerTimeMeanNOneTwenty}{92}
\newcommand{\SemmlSemmlFastAigerTimeWtoMeanNZero}{1392}
\newcommand{\SemmlSemmlFastAigerTimeWtoMeanNFive}{704}
\newcommand{\SemmlSemmlFastAigerTimeWtoMeanNTen}{416}
\newcommand{\SemmlSemmlFastAigerTimeWtoMeanNThirty}{205}
\newcommand{\SemmlSemmlFastAigerTimeWtoMeanNOneTwenty}{108}
\newcommand{\SemmlSemmlFastAigerSizeMeanTotal}{0.58}
\newcommand{\SemmlSemmlFastAigerSizeMeanReal}{0.58}
\newcommand{\SemmlSemmlFastAigerSizeMeanNTotal}{603}
\newcommand{\SemmlSemmlFastAigerSizeMeanNReal}{603}
\newcommand{\SemmlLtlsyntAigerUniqueSolvesTotal}{188}
\newcommand{\SemmlLtlsyntAigerUniqueSolvesReal}{123}
\newcommand{\SemmlLtlsyntAigerUniqueSolvesUnreal}{65}
\newcommand{\LtlsyntSemmlAigerUniqueSolvesTotal}{26}
\newcommand{\LtlsyntSemmlAigerUniqueSolvesReal}{24}
\newcommand{\LtlsyntSemmlAigerUniqueSolvesUnreal}{2}
\newcommand{\SemmlLtlsyntAigerSolvesBoth}{1187}
\newcommand{\SemmlLtlsyntAigerSolvesNeither}{162}
\newcommand{\SemmlLtlsyntAigerTimeMeanZero}{25.92}
\newcommand{\SemmlLtlsyntAigerTimeMeanFive}{8.71}
\newcommand{\SemmlLtlsyntAigerTimeMeanTen}{3.19}
\newcommand{\SemmlLtlsyntAigerTimeMeanThirty}{1.15}
\newcommand{\SemmlLtlsyntAigerTimeMeanOneTwenty}{1.13}
\newcommand{\SemmlLtlsyntAigerTimeWtoMeanZero}{11.23}
\newcommand{\SemmlLtlsyntAigerTimeWtoMeanFive}{2.48}
\newcommand{\SemmlLtlsyntAigerTimeWtoMeanTen}{0.72}
\newcommand{\SemmlLtlsyntAigerTimeWtoMeanThirty}{0.26}
\newcommand{\SemmlLtlsyntAigerTimeWtoMeanOneTwenty}{0.17}
\newcommand{\SemmlLtlsyntAigerTimeFacZero}{0.04}
\newcommand{\SemmlLtlsyntAigerTimeFacFive}{0.11}
\newcommand{\SemmlLtlsyntAigerTimeFacTen}{0.31}
\newcommand{\SemmlLtlsyntAigerTimeFacThirty}{0.87}
\newcommand{\SemmlLtlsyntAigerTimeFacOneTwenty}{0.89}
\newcommand{\SemmlLtlsyntAigerTimeWtoFacZero}{0.09}
\newcommand{\SemmlLtlsyntAigerTimeWtoFacFive}{0.40}
\newcommand{\SemmlLtlsyntAigerTimeWtoFacTen}{1.40}
\newcommand{\SemmlLtlsyntAigerTimeWtoFacThirty}{3.85}
\newcommand{\SemmlLtlsyntAigerTimeWtoFacOneTwenty}{5.79}
\newcommand{\SemmlLtlsyntAigerTimeMeanNZero}{1187}
\newcommand{\SemmlLtlsyntAigerTimeMeanNFive}{533}
\newcommand{\SemmlLtlsyntAigerTimeMeanNTen}{292}
\newcommand{\SemmlLtlsyntAigerTimeMeanNThirty}{152}
\newcommand{\SemmlLtlsyntAigerTimeMeanNOneTwenty}{76}
\newcommand{\SemmlLtlsyntAigerTimeWtoMeanNZero}{1401}
\newcommand{\SemmlLtlsyntAigerTimeWtoMeanNFive}{747}
\newcommand{\SemmlLtlsyntAigerTimeWtoMeanNTen}{498}
\newcommand{\SemmlLtlsyntAigerTimeWtoMeanNThirty}{358}
\newcommand{\SemmlLtlsyntAigerTimeWtoMeanNOneTwenty}{282}
\newcommand{\SemmlLtlsyntAigerSizeMeanTotal}{0.24}
\newcommand{\SemmlLtlsyntAigerSizeMeanReal}{0.24}
\newcommand{\SemmlLtlsyntAigerSizeMeanNTotal}{480}
\newcommand{\SemmlLtlsyntAigerSizeMeanNReal}{480}
\newcommand{\RealSolvedByAllInFiveSec}{749}
\newcommand{\RealSolvedByAllInTenSec}{924}
\newcommand{\RealSolvedByAllInOneMin}{1117}
\newcommand{\RealSolvedByAllInThirtyMin}{1240}
\newcommand{\RealSolvedByNoneInFiveSec}{426}
\newcommand{\RealSolvedByNoneInTenSec}{363}
\newcommand{\RealSolvedByNoneInOneMin}{221}
\newcommand{\RealSolvedByNoneInThirtyMin}{128}
\newcommand{\MealySolvedByAllInFiveSec}{667}
\newcommand{\MealySolvedByAllInTenSec}{859}
\newcommand{\MealySolvedByAllInOneMin}{1040}
\newcommand{\MealySolvedByAllInThirtyMin}{1164}
\newcommand{\MealySolvedByNoneInFiveSec}{481}
\newcommand{\MealySolvedByNoneInTenSec}{421}
\newcommand{\MealySolvedByNoneInOneMin}{273}
\newcommand{\MealySolvedByNoneInThirtyMin}{175}
\newcommand{\AigerSolvedByAllInFiveSec}{420}
\newcommand{\AigerSolvedByAllInTenSec}{737}
\newcommand{\AigerSolvedByAllInOneMin}{1005}
\newcommand{\AigerSolvedByAllInThirtyMin}{1132}
\newcommand{\AigerSolvedByNoneInFiveSec}{497}
\newcommand{\AigerSolvedByNoneInTenSec}{419}
\newcommand{\AigerSolvedByNoneInOneMin}{271}
\newcommand{\AigerSolvedByNoneInThirtyMin}{159}


==> preamble/0_macros.tex <==


\RequirePackage{amsmath}
\RequirePackage{amssymb}


\RequirePackage{marvosym}
\providecommand{\contradiction}{\Lightning}


\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\pospart}{\lgroup}{\rgroup^+}
\DeclarePairedDelimiter{\negpart}{\lgroup}{\rgroup^-}
\DeclarePairedDelimiterX{\inner}[2]{\lange}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\cardinality}{\lvert}{\rvert}
\DeclarePairedDelimiter{\set}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\tuple}{(}{)}
\DeclarePairedDelimiter{\listt}{[}{]}



\newcommand{\setcomplement}[1]{{#1}^c}
\newcommand{\powerset}[1]{\mathcal{P}(#1)}

\newcommand{\unionSym}{\cup}
\newcommand{\unionBin}{\mathbin{\unionSym}}
\newcommand{\strictunionSym}{\dot{\unionSym}}
\newcommand{\strictunionBin}{\mathbin{\dot{\unionSym}}}
\newcommand{\intersectionSym}{\cap}
\newcommand{\intersectionBin}{\mathbin{\intersectionSym}}
\newcommand{\UnionSym}{\bigcup}
\newcommand{\UnionBin}{\mathbin{\UnionSym}}
\newcommand{\strictUnionSym}{\dot{\UnionSym}}
\newcommand{\strictUnionBin}{\mathbin{\strictUnionSym}}
\newcommand{\IntersectionSym}{\bigcap}
\newcommand{\IntersectionBin}{\mathbin{\IntersectionSym}}

\newcommand{\union}{\unionBin}
\newcommand{\strictunion}{\strictunionBin}
\newcommand{\intersection}{\intersectionBin}
\newcommand{\Union}{\UnionSym}
\newcommand{\strictUnion}{\strictUnionSym}
\newcommand{\Intersection}{\IntersectionSym}



\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Rationals}{\mathbb{Q}}
\newcommand{\Reals}{\mathbb{R}}



\newcommand{\gradient}{\nabla}
\newcommand{\laplacian}{\Delta}
\newcommand{\diff}{\partial}
\newcommand{\boundary}{\partial}
\DeclareMathOperator{\divergence}{div}
\DeclareMathOperator{\distance}{dist}
\DeclareMathOperator{\esssup}{ess sup}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\capacity}{cap}
\DeclareMathOperator{\signum}{signum}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator*{\argmin}{arg\, min}

\newcommand{\qee}{\hfill$\triangle$} %


\newcommand{\lOr}{\bigvee}
\newcommand{\lAnd}{\bigwedge}
\newcommand{\lfalse}{\texttt{ff}}
\newcommand{\ltrue}{\texttt{tt}}

\DeclareMathOperator{\ExistsOp}{\exists}
\DeclareMathOperator{\ForallOp}{\forall}

\newcommand{\LTL}{\operatorname{LTL}}
\newcommand{\CTL}{\operatorname{CTL}}
\newcommand{\PCTL}{\operatorname{pCTL}}

\newcommand{\ltlNext}{\operatorname{\mathbf{X}}}
\newcommand{\ltlFinally}{\operatorname{\mathbf{F}}}
\newcommand{\ltlGlobally}{\operatorname{\mathbf{G}}}
\newcommand{\ltlUntil}{\mathbin{\mathbf{U}}}
\newcommand{\ltlWuntil}{\mathbin{\mathbf{W}}}
\newcommand{\ltlRelease}{\mathbin{\mathbf{R}}}
\newcommand{\ltlSrelease}{\mathbin{\mathbf{M}}}
\newcommand{\ltlLanguage}[1]{\mathcal{L}(#1)}
\newcommand{\true}{\texttt{tt}}
\newcommand{\false}{\texttt{ff}}
\newcommand{\trueness}{t}

\newcommand{\Alphabet}{\Sigma}
\newcommand{\AP}{\mathsf{AP}}

\DeclareMathOperator{\subformulas}{sub}
\DeclareMathOperator{\topformulas}{top}

\DeclareMathOperator{\satisfying}{sat}


\newcommand{\NP}{\mathbf{NP}}
\newcommand{\coNP}{\mathbf{coNP}}
\newcommand{\NEXP}{\mathbf{NEXP}}
\newcommand{\PSPACE}{\mathbf{PSPACE}}


\newcommand{\G}{\mathcal{G}}
\newcommand{\Vertices}{V}
\newcommand{\Edges}{E}
\newcommand{\VertexPlayer}{P}
\newcommand{\EdgesSys}{E_\sys}
\newcommand{\EdgesEnv}{E_\env}
\newcommand{\initialvertex}{v_0}
\newcommand{\play}{\rho}
\newcommand{\Plays}{\mathfrak{P}}
\newcommand{\player}{p}
\newcommand{\strategy}{\sigma}
\newcommand{\priorities}{\mathfrak{p}}

\newcommand{\sys}{\mathcal{S}}
\newcommand{\env}{\mathcal{E}}
\newcommand{\VerticesSys}{\Vertices_\sys}
\newcommand{\VerticesEnv}{\Vertices_\env}

\newcommand{\GExt}{\mathsf{Ext}}

\DeclareMathOperator{\obligationSetFormula}{\emph{osf}}
\DeclareMathOperator{\someAssignment}{\mathcal{A}}

\newcommand{\smallenv}{\mathsf{ENV}}%
\newcommand{\smallsys}{\mathsf{SYS}}%

\newcommand{\para}[1]{\paragraph{#1}}

\input{data/commands.tex}

\newcommand{\SemML}{\textsc{SemML}}
\newcommand{\SemMLOne}{\textsc{SemML}$_{1.0}$}
\newcommand{\SemMLTwo}{\textsc{SemML}$_{2.0}$}
\newcommand{\SemMLTwoF}{\textsc{SemML2F}}
\newcommand{\Strix}{\textsc{Strix}}
\newcommand{\ltlsynt}{\textsc{ltlsynt}}
\newcommand{\spot}{\textsc{Spot}}
\newcommand{\Owl}{\textsc{Owl}}
\newcommand{\LtlSynt}{\textsc{LtlSynt}}
\newcommand{\Syntcomp}{\textsc{SYNTCOMP}}
\newcommand{\Neurosynt}{\textsc{NeuroSynt}}

\newcommand{\runReal}{\textsf{Real}}
\newcommand{\runMealy}{\textsf{Mealy}}
\newcommand{\runAiger}{\textsf{Aiger}}

\newcommand{\envvar}[1]{\ensuremath{x_{#1}}}
\newcommand{\sysvar}[1]{\ensuremath{y_{#1}}}

\newcommand{\Sum} [2] {\the\numexpr #1 + #2 \relax}
\newcommand{\Diff} [2] {\the\numexpr #1 - #2 \relax}

